Smartphone Impostor Detection with Built-in Sensors and Deep Learning

In this paper, we show that sensor-based impostor detection with deep learning can achieve excellent impostor detection accuracy at lower hardware cost compared to past work on sensor-based user authentication (the inverse problem) which used more conventional machine learning algorithms. While these methods use other smartphone users' sensor data to build the (user, non-user) classification models, we go further to show that using only the legitimate user's sensor data can still achieve very good accuracy while preserving the privacy of the user's sensor data (behavioral biometrics). For this use case, a key contribution is showing that the detection accuracy of a Recurrent Neural Network (RNN) deep learning model can be significantly improved by comparing prediction error distributions. This requires generating and comparing empirical probability distributions, which we show in an efficient hardware design. Another novel contribution is in the design of SID (Smartphone impostor Detection), a minimalist hardware accelerator that can be integrated into future smartphones for efficient impostor detection for different scenarios. Our SID module can implement many common Machine Learning and Deep Learning algorithms. SID is also scalable in parallelism and performance and easy to program. We show an FPGA prototype of SID, which can provide more than enough performance for real-time impostor detection, with very low hardware complexity and power consumption (one to two orders of magnitude less than related performance-oriented FPGA accelerators). We also show that the FPGA implementation of SID consumes 64.41X less energy than an implementation using the CPU with a GPU.

==> 0100_introduction.tex <==
\section{Introduction}

%To prevent potential abuse of the smartphone during a theft by an anomalous user, sensor-based detection has been proposed as a supplement to traditional authentication methods e.g. the password. However, many detection methods are based on machine learning and deep learning models whose training requires other user or potential attacker's data. It remains unknown whether a detection algorithm can defeat attackers using only the real user's data and how to design a hardware module that can support the whole detection process.

%This paper presents the functional primitives needed for sensor-based impostor detection by studying a set of machine learning/deep learning algorithms. We identify the possibility to enhance a one-class model with the statistic test. We design a lightweight programmable hardware module to execute the detection algorithms with least hardware cost. We further propose hardware features to save the cost of control while increase its flexibility. The evaluation shows the one-class model can achieve both comparable accuracy and performance to multi-class models.

%The anomalous user is the malicious people who takes control of a victim's electronic device and tries to steal his/her confidential information or do malicious behaviors. To prevent potential abuse of the smartphone, sensor-based detection has been proposed as a supplement to traditional authentication methods e.g. the password. While many detection mechanisms are based on machine learning and deep learning algorithms, how they can be supported by existing deep learning accelerators remains unknown. 

%This paper presents the software and hardware design primitives needed for sensor-based impostor detection by studying a set of machine learning/deep learning algorithms. We identify the possibility to build one-class models and the improvement by introducing frequency-domain features. We design a lightweight programmable hardware module to execute the detection algorithms with least hardware cost. Based on the baseline, we propose some HW features for flexible control. We evaluate the models for real-time detection from both software and hardware perspectives.

Machine learning (ML) and deep learning techniques (DL) have become widely used for data analysis for various purposes in the real world. To support the computation and memory intensive deep learning computation, specialized accelerators have been studied for certain commonly used deep network architecture such as convolutional neural network (CNN) and recurrent neural network (RNN). These model-specific accelerators (MSA) are designed with the knowledge of the certain model and can thus leverage techniques like data reuse and data sparsity to deliver higher performance or energy efficiency than the general-purpose computing devices. %The accelerators also avoid including the hardware resources that are designed for general-purpose computation but don't have much advantage

However, the data analysis in the real world is not always so simple that one specific model can fulfill the analysis task in all cases. In one application, different ML and DL models can be needed depending on the actual user case. It is also possible that the output of a model needs subsequent processing for better final results. If a specialized MSA is used, there are difficulties when the application has to switch to another model that the MSA cannot support or it has to transmit its results back to general-purpose computing devices for subsequent processing.

%These cases pose challengers for 

When the accelerators are built to optimize the trade-off between computation efficiency and design cost, there are two directions from the function perspective in which they can proceed to overcome the limitation of MSAs. The first one is to still pursue maximum power efficiency when the system, e.g. the cloud computing center, is not sensitive to the size or kinds of accelerators that will be used. The system designer can provide versatility by integrating multiple MSAs dedicated to different network architectures. The second direction is designing a versatile accelerator for models that will potentially be used. This direction is important for the Internet of things (IoT) or embedded systems because they are usually resource-constraint and not able to incorporate multiple MSAs. On the other hand, IoT or embedded systems always have a fixed range of functionality so that hardware designers can explore prior knowledge to decide the level of versatility.

% from 0400_module.tex
% We want to design a detection module that is versatile to support the analysis for impostor detection in difference user cases. The module should be able to have a standalone runtime for impostor detection, which means it can give a yes-or-no answer without any subsequent processing on other devices. 

We explore in the second direction and identify three critical challenges to build a hardware module that provides support for the entire analysis and produces the final result without the need for subsequent processing. These challenges make directly integrating %the performance and efficiency oriented 
MSAs infeasible for versatile data analysis. 
\begin{itemize}
    \item Challenge 1: %\newline
    A real application can require different ML/DL models depending on the real use cases.
    \item Challenge 2:
    A real application can apply auxiliary data processing techniques which gets processed after or even between model inference.
    \item Challenge 3:
    A real application can involve the control flow having various layers of loops
\end{itemize}

%We explore in the second direction to get prior knowledge about the algorithms that can potentially be used and 

We propose an algorithm-hardware exploration methodology to design a minimalist but versatile hardware module using the example of impostor detection. 

Smartphones are one of the most frequently used mobile devices that people use in their daily life. Users store their confidential information such as photos and videos in the smartphones. The smartphone is also used for remote access by financial or social applications. The impostor is the kind of attacker who controls the smartphone by stealing or cheating and pretends to be the real user. All the security properties of critical applications in the smartphone are threatened by the potential abuse from impostors. Therefore it is important to authenticate a user before a sensitive usage.

Explicit authentication such as password and PINs has been integrated into smartphones to prevent potential impostors from using the smartphone. Biometric-based authentication is also implemented in real smartphone using fingerprint~\cite{clancy2003secure} or facial information~\cite{jafri2009survey}. However, these protection mechanisms are all one-time checks. It is possible for an attacker to take control of the phone after the real user passes the primary authentication.

Sensor-based user authentication~\cite{lee2017implicit} has then been proposed as a second defense in addition to the primary authentication. The authentication system collects the readings from sensors like the accelerometer and the gyroscope which are built into typical smartphones. The system contains a machine learning model that is trained off-line with multiple users' data to distinguish the real user from others. With the model, the system is able to implicitly read the sensors and authenticate the user without explicitly asking for the user's input.

However, there are still problems when a machine learning (ML) or deep learning (DL) model is deployed for sensor-based impostor detection. The continuous detection on sensor readings causes periodic interruptions to the applications running on the smartphone processor and have a negative impact on user experience. A dedicated hardware impostor module is needed but existing performance oriented accelerators may not have the functional support for the whole analysis and require subsequent processing or they are over-designed to be too gigantic to fit in the smartphone and work under the power constraint of the sleep mode.
%An alternative is to design a lightweight hardware module implementing only the necessary functional units for ML/DL models. 
Therefore, we develop a methodology to design a lightweight hardware module on FPGA implementing only the necessary functional units for ML/DL models with the goal to provide enough performance using the least amount hardware resources and power consumption.

The methodology consists of two main steps. In the first step, we explore the necessary ML/DL models and auxiliary processing techniques by evaluating their accuracy. We leverage the prior knowledge of use cases and decide what models and techniques are useful in each case and should be supported by the module for impostor detection. In the second step, we decompose the models and processing techniques into a set of computation primitives. We then build a minimalist module,~\modulename, that is able to support the necessary primitives. We also consider the control flow of nested loops involved in some algorithms and provide relevant hardware support.

%The background of several ML/DL models is detailed in~\gyrefsec{sec_background}. 
We present what models and auxiliary processing techniques are in different scenarios of impostor detection in~\gyrefsec{sec_sw_model}. We show how our~\modulename~module for self-contained impostor detection which is designed with the knowledge of selected algorithms and the goal to save hardware utilization and power consumption in~\gyrefsec{sec_hw}. The evaluation is given in~\gyrefsec{sec_evaluation}.~\gyrefsec{sec_related_work} contains the relationship with previous work. The whole paper is concluded in~\gyrefsec{sec_conclusion}.

\iffalse
The main contributions of this paper are:
\begin{packeditemize}

\item We summarize a set of ML/DL algorithms for impostor detection. In addition to conventional binary classification models which require other users' data for training, we investigate the model for time-series modeling to enable one-class training.

\item We identify the fundamental operation primitives needed by relevant ML/DL algorithms.



\item We show a novel lightweight and scalable implementation of a programmable hardware module for ML/DL that implements these primitives.

\item We evaluate the ML/DL models for real-time impostor detection in terms of accuracy, execution time and memory usage.

\item We define an algorithm-HW methodology that determines the best security-performance trade-off for a resource-constraint device,

\end{packeditemize}
\fi


==> 0101_intro_new_hpca.tex <==
\section{Introduction}

We rely heavily on our smartphones not only for communication but also to store our private information and access remote cloud services. This means a lot of confidential and sensitive data will be lost if smartphone theft happens\cite{wang2012smartphonetheft}. An impostor is defined as an adversary who gets hold of a smartphone that does not belong to him. The impostor may try to access information and services that he is not authorized to access, but the legitimate user of the smartphone is authorized to access. Hence, implicit impostor detection mechanism built into the smartphone would make stealing smartphones less attractive if the smartphone detects the impostor, and prevents access, at least to secret and sensitive material. Ideally, we would like to detect a potential impostor even before he/she tries to access any secret or sensitive data, code or services. Is it feasible to detect an impostor as he is just walking with the smartphone?

To solve this important security problem of smartphone impostor detection, or theft deterrence, we leverage two new opportunities in the computing landscape today: the ubiquitous inclusion of motion sensors in smartphones and the rise of deep learning algorithms. We will use both synergistically in our solution.

Built into all smartphones today is a sensor subsystem that comprises motion sensors and other sensors like light, barometer, magnetometer, etc. The most common sensors are the 3-axis accelerometer and the 3-axis gyroscope, which are found in almost all smartphones and smartwatches, not just the high-end ones. The readings from these sensors are not considered privacy-sensitive, unlike the GPS which gives the location, or cameras and microphones, which can divulge private scenes or conversations. We use data from these two widely-available sensors to characterize the motion of the person currently holding the smartphone, as he is walking away from the theft scene, etc. Past work has succeceed in using such sensors to implicitly and continuously authenticate a user\cite{lee2017implicit}. It seems that physiological behavior, like how a person walks or holds a smartphone can be captured by time-series measurements of an accelerometer or gyroscope, and analyzed by advanced algorithms.

For these sensor-based authentication systems, traditional Machine Learning (ML) algorithms like Support Vector Machine (SVM) and Kernel Ridge Regression (KRR) have been proposed. The rise of Deep Learning (DL) algorithms, where there is no need to first compute heuristically derived features, is an attractive alternative. Toward detecting the impostors, we consider two different user scenarios. In the first scenario, users subscribe to an "impostor Detection as a Service (IDaaS)". They register to a service and obtain a trained ML or DL model on their smartphone for subsequent real-time impostor detection. That model is trained with both the legitimate user's sensor data and the sensor data from other users of the IDaaS service. In the second scenario, users are more privacy-shy and do not want to send their sensor data to a cloud service. Their ML or DL model is trained locally, with only the legitimate user's sensor data. We show that there exists an important trade-off between the detection accuracy (usability) and the increased privacy of the user's sensor data.

Modern smartphones are equipped with various computation subsystems dedicated to different application domains\cite{hexagon:2014micro:codrescu2014hexagon}. For the domain of impostor detection, we investigate whether a small and energy-efficient hardware module for impostor detection can be designed for the self-contained computation. Unlike previous work on ML/DL accelerators whose goal is to get the maximum performance from one or a few specific ML or DL algorithms, like Convolutional Neural Networks (CNN), leveraging data reuse~\cite{diannao:Chen:2014:DSH:2541940.2541967}\cite{eyeriss2016isca} or matrix sparsity features\cite{han2016eie}, our goal is not to maximize performance, but sufficient performance at small size and low power consumption. Past work also looked at maximizing the energy efficiency of certain Deep Neural Network (DNN) accelerators, but this is different from our goal to pursue the minimal energy consumption.

We design Smartphone impostor Detection Engine (SIDE) to show that we can efficiently and effectively solve a real security problem (small hardware footprint and energy consumption). We call this architecture \modulename~for Smartphone impostor Detection engine. \modulename~reuses functional units where possible to reduce size and cost. Yet it is also scalable for higher performance if more parallel datapath tracks are implemented. It is designed to support not only the best deep learning algorithms we found for impostor detection in both user scenarios, but can also support other Machine Learning algorithms, calculations of empirical probability distributions and statistical tests. Programmability support provides flexibility in the choice of algorithms.

Our key contributions are:
\begin{packeditemize}

\item Investigating a comprehensive comparison of Machine Learning and Deep Learning algorithms for two user scenarios of impostor detection, where other people's data are used, or not used, in the training phase, trading off detection accuracy versus data privacy.

\item Achieving over 96\% accuracy in impostor detection for the IDaaS user scenario (2-class models), and over 88\% accuracy in the single-user scenario (1-class models).

\item Proposing~\modulename~ module that is versatile, scalable and efficient to perform self-contained impostor detection without subsequent processing on other devices.

\item Showing the trade-off between detection accuracy with performance and energy consumption when models are mapped to the~\modulename~module.

\item Showing a major difference in size between the~\modulename~module and existing accelerators with a similar target.

\item Showing SIDE uses 64.4X less energy than a server platform with a GPU

\end{packeditemize}

==> 0200_background.tex <==
\section{Background}
\label{sec_background}

%\subsection{Sensor-based Impostor Detection}

\subsection{Multi-class Models}
\label{sec_model_class}

We consider representative ML/DL models to classify a sample of sensor data as being the real user or a potential impostor. Logistic regression intrinsically provides the probability of a class, and thus can be naturally leveraged as the warning score. KRR alleviates over-fitting by penalizing large parameters. It is suitable for learning with limited data. We evaluate SVM because it is a light-weight and powerful linear model. MLP is a non-linear classifier and can automatically extract complex patterns from raw data, without heuristic and tedious hand-crafting.

\bheading{Regression}
Regression is a model describing the linear relationship between the input and the output. In the context of impostor detection, we use the logistic regression whose output could be treated as a probability for predicting whether a smartphone is currently under the control of an attacker. The computation for inference of a linear regression model is given in \gyrefeq{eq_linearreg}. 
\begin{equation}
\label{eq_linearreg}
  Y = W \times x_{input} + b
\end{equation}

The logistic regression produces its output by applying an additional non-linear logistic function as shown in \gyrefeq{eq_logisreg}. The logistic function is actually converting a real number to an output between 0 and 1 which can be treated as a probability.
\begin{equation}
\label{eq_logisreg}
  Y = f(W \times x_{input} + b), where f(z) = \frac{1}{1+e^{-z}}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./figures/svm_fig.pdf}
    \caption{The optimal hyperplane in SVM}
    \label{img_svm}
\end{figure}

\bheading{Support Vector Machine} The support vector machine (SVM) is one of the most commonly used models in machine learning. To perform a binary classification, it identifies a hyperplane in a high-dimensional space as the decision boundary. As shown in \gyreffig{img_svm}, the SVM model is trained to find the optimal hyperplane (the green line) which maximizes the margin between data points from two classes. It is provable~\cite{wiki:svm} that the optimal hyperplane can be decided by a set of support vectors sitting on the maximized margin in the data plane.
%the trained parameter $\vec{w}$ and $b$ and consists of all the data points which makes Y equal to 0 in \gyrefeq{eq_svm}.~\cite{wiki:svm}

In the inference phase, \gyrefeq{eq_svm} is computed for testing samples. In~\gyrefeq{eq_svm}, there are $n\_sv$ support vectors, namely $\vec{x_i}$'s. $c_i$'s are coefficients obtained in the training phase. $y_i$ is either $1$ or $-1$ depending on which side of the hyperplane the support vector resides on. The angle bracket stands for the inner product of the input testing sample, $\vec{x_{input}}$, and a support vector. The class of the testing sample is decided by the sign of Y.%, which actually decides which side of the hyperplane the input resides on. 
\begin{equation}
  Y = \sum^{n\_sv}_{i=1} c_i y_i \langle \vec{x_i}, \vec{x_{input}} \rangle + b%, where~\vec{w} = 3
\label{eq_svm}
\end{equation}

To enable more flexible separation with a curve boundary, the inner product of $\vec{w}$ and $\vec{x_{input}}$ could be replaced by kernel functions, e.g. the Gaussian kernel in~\gyrefeq{eq_svm_kernel}. The use of kernel functions represents the inner product when the data points are projected into a higher-dimensional space so that a non-linear separation is made possible.
\begin{equation}
  \begin{split}
    &Y = \sum^{n\_sv}_{i=1} c_i y_i \kappa(\vec{x_i}, \vec{x_{input}}) + b \\
    &\kappa(\vec{x}, \vec{y}) = e^{- \gamma \norm{\vec{x}-\vec{y}}^2}
  \end{split}
\label{eq_svm_kernel}
\end{equation}

\bheading{Multilayer Perceptron}

Neural network (NN) models have been used for deep learning. Multilayer perceptron (MLP) is a basic feedforward NN model which contains at least three layers of neurons. The first layer of neurons is the input layer which collects the input data. The last layer is the output layer presenting the final results. Between the input and the output layer are the hidden layers and the depth of a NN is decided by the number of hidden layers. In the feedforward path, the neurons in the next layer is obtained by applying linear transformation and then non-linear activation functions to the neurons in the previous layer. The weight and bias used in the linear transformation are trainable with gradient descent and back-propagation. In the inference phase described in ~\gyrefeq{eq_mlp}, $W$'s and $b$'s are trained weight matrices and bias vectors superscripted with the layer index $l$. 
\begin{equation}
\centering
\begin{split}
  &x^0 = x_{input} \\
  &x^{l+1} = f(W^l \times x^l + b^l)%, where f(z) is the activation function
\end{split}
\label{eq_mlp}
\end{equation}

\subsection{Models for Time-Series Modeling}
\label{sec_model_time}

Deep learning models are also studied to model time-series. One usage of the model is to predict the incoming data based on the past observations. While the prediction can be directly used by forecasting applications, it is also feasible to detect anomalies by calculating the prediction error. If a model is assumed to represent the time-series generated by a certain subject, a high prediction error when predicting with this model will indicate an anomalous series or even a potential ongoing attack.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./figures/lstm_fig.pdf}
    \caption{The computations within a LSTM cell}
    \label{img_lstm}
\end{figure}

Long short-term memory (LSTM) has been proposed as a variant of recurrent neural network (RNN) to learn long-term dependency and avoid the problem of vanishing gradient~\cite{bengio1994learning}. Different from the stateless models mentioned in~\gyrefsec{sec_model_class}, the LSTM model has two hidden states (h state and c state) which can remember the previous input information.

When analyzing a series, a LSTM cell will update its hidden states for each input element as described in~\gyrefeq{eq_lstm} and ~\gyreffig{img_lstm}. In~\gyrefeq{eq_lstm}, the W's and U's are weight matrices, the b's are bias vectors and $x_t$ is the input feature vector at time t. Conceptually, with the previous h state $h_{t-1}$ and the input $x_t$, the LSTM cell first computes $cand_t$ as a candidate for new c state and three control gates, the forget gate $f_t$, the input gate $i_t$ and the output gate $o_t$. The new c state $c_t$ is then computed as a sum of old c state $c_{t-1}$ and $cand_t$ weighted by $f_t$ and $i_t$ respectively. The new h state $h_t$ is generated from $o_t$ and the new $c_t$.
\begin{equation}
\begin{split}
  &cand_t = tanh(W_c \times x_{t} + U_c \times h_{t-1} + b_c) \\
  &f_t = \sigma (W_f \times x_{t} + U_f \times h_{t-1} + b_f) \\
  &i_t = \sigma (W_i \times x_{t} + U_i \times h_{t-1} + b_i) \\
  &o_t = \sigma (W_o \times x_{t} + U_o \times h_{t-1} + b_o) \\
  &c_t = f_t \odot c_{t-1} + i_t \odot cand_t \\%, where f(z) is the activation function
  &h_t = o_t \odot tanh(c_t)
\end{split}
\label{eq_lstm}
\end{equation}



==> 0402_macro.tex <==
%\subsection{Instruction Encoding}
\subsection{Flexible Storage and Control}
\label{sec_inst_enc}

==> 040601_loop_support.tex <==
%\subsection{Nested Loop Support}
\subsection{Software-Hardware Nested Loop Support}
\label{sec_loop_support}

Although a macro instruction can perform the innermost loop operations on vector and/or matrix operands, often there are multiple nested loops that must be performed, e.g., in computing the kernel function in an SVM model for each support vector (\gyrefapd{apd_class_alg}). To avoid increasing the code size linearly with the number of iterations, we propose \textbf{\modulename +}, which is the \modulename~module with the extension to do nested loops efficiently. In \textbf{\modulename +}, the software program is responsible for managing the nested loop control information including the loop state and the address offsets to load/store an operand using four new instructions (\textbf{Loop}, \textbf{RegAddi}, \textbf{RegStore} and \textbf{RegLoad}).

The loop state is determined by three newly added registers, \textbf{loop\_be\-gin},~\textbf{lo\-op\_e\-nd} and~\textbf{lo\-op\_n}, which store the current loop's beginning PC, end PC and the number of unfinished iterations respectively. They are initialized when a~\textbf{Loop} instruction is executed. The hardware assumes that the loop will start after the~\textbf{Loop} instruction and sets~\textbf{loop\_end} and~\textbf{lo\-op\_n} to \textbf{inst[95:64]} and \textbf{inst[63:32]} respectively. When the program counter reaches \textbf{loop\_end}, the hardware checks~\textbf{loop\_n} and jumps back to the beginning of the loop if there are iterations that have not been finished.

We enable data accesses to different addresses by adding three address offset registers to access the operands (two input operands and one output operand) used in different iterations. The offset enable bits in the macro instruction, e.g.~\textbf{Off\_X} in~\gyreftbl{tbl_inst_fmt}, decides whether an address offset is added to the base address. To increase the address offset after each iteration, we support adding an immediate number to an address offset register using the~\textbf{RegAddi} instruction.

For a nested loop with multiple loop layers, we add two instructions,~\textbf{RegStore} and~\textbf{RegLoad}, to save and restore the loop state registers. In a nested loop, the external loop saves its loop state and address offsets before entering the inner loop and restores them after the inner loop exits.

\input{0604_loop_code_reduction.tex}

==> 0406_loop_support.tex <==
%\subsection{Nested Loop Support}
\subsection{Software-Hardware Nested Loop Support}
\label{sec_loop_support}

Although a macro instruction can perform the innermost loop operations on vector and/or matrix operands, often there are multiple nested loops that must be performed, e.g., in computing the kernel function in an SVM model for each support vector (\gyrefapd{apd_class_alg}). The straightforward way to fulfill a nested loop is repeating the macro instructions and manually specifying the operands in each iteration. However, this will make the code size scale linearly with the number of iterations% and become an unacceptable overhead for storage-constrained mobile devices
. We propose \textbf{\modulename +}, which is the \modulename~module with the extension to do nested loops in a flexible and efficient way. We identify the necessary loop control information (loop states and the address offsets to load/store an operand) and provide the ability to save/restore the loop state and address offsets. In \textbf{\modulename +}, the software program is responsible for managing the nested loop controls, and four new instructions (\textbf{Loop}, \textbf{RegAddi}, \textbf{RegStore} and \textbf{RegLoad}).%loop termination counters for each level of looping, saving these before going to the next higher or lower loop level, and restoring them when returning to this loop level.

\iffalse
%Encoding a one-layer loop of homogeneous operations in a macro instruction is not enough when a nested loop of multiple layers is involved or a loop contains multiple heterogeneous operations. 
For instance, the inference of a Gaussian kernel based SVM requires multiple kinds of vector operations for each support vector (\gyrefsec{sec:service:alg}). The straightforward way to fulfill a nested loop is repeating the macro instructions and manually specifying the operands in each iteration
. However, this will make the code size scale linearly with the number of iterations% and become an unacceptable overhead for storage-constrained mobile devices
. We enable a flexible nested loop control by identifying the necessary loop control information (loop states and the address offsets to load/store an operand) and providing the ability to save/restore the loop state and address offsets. 
\fi

The loop state is determined by three newly added registers, \textbf{loop\_be\-gin},~\textbf{lo\-op\_e\-nd} and~\textbf{lo\-op\_n}, which store the current loop's beginning PC, end PC and the number of unfinished iterations respectively. They are initialized when a~\textbf{Loop} instruction is executed. The hardware assumes that the loop will start after the~\textbf{Loop} instruction and sets~\textbf{loop\_end} and~\textbf{lo\-op\_n} to the numbers encoded in the~\textbf{Loop} instruction as shown in~\gyreflst{alg_loop_control}. The three registers then control the loop execution by deciding whether \modulename~needs to jump back to the beginning of the loop. When a loop reaches the end, the hardware checks~\textbf{loop\_n} and jumps back to the beginning of the loop if there are iterations that have not been finished.
\begin{lstlisting}[language=C,
%frame=single,
xleftmargin=.5em, framexleftmargin=.5em, caption={Loop States}, label={alg_loop_control}]
    Init: Registers are set by a loop instruction
  	  // The loop starts from the next instruction
      loop_begin <- PC(loop) + 1 
      loop_end   <- inst[95:64]
      loop_n     <- inst[63:32]
    Execution:
      if (PC == loop_end) && (loop_n != 0)
        // jump back to the beginning of the loop
        PC     <- loop_begin
        loop_n <- loop_n - 1
\end{lstlisting}

The address offsets are needed for incremental data access as iterations may need to access multiple operands in a row, e.g. support vectors in an SVM model. We enable this feature by adding three address offset registers to access the operands (two input operands and one output operand). The address generation logic decides whether each address offset is added to the corresponding address depending on the offset enable bits encoded in the current macro instruction, e.g.~\textbf{Off\_X} in~\gyreftbl{tbl_inst_fmt}. To increase the address offset properly after each iteration, we support adding an immediate number to an address offset register using the~\textbf{RegAddi} instruction.

For a single-layer loop, the loop control registers and address offset registers define the current loop state. %However, more layers of loops can be involved due to the need to process multiple data samples or more complex models. 
For a nested loop with multiple loop layers, we add two instructions,~\textbf{RegStore} and~\textbf{RegLoad}, to save and restore the loop state registers. In a nested loop, the external loop saves its loop state and address offsets before entering the inner loop and restores them after the inner loop exits.~\gyreflst{alg_nested_loop} shows the pseudo-code of an example two-layer loop.
\begin{lstlisting}[language=C,
%frame=single,
xleftmargin=.5em, framexleftmargin=.5em, caption={Save/restore loop state registers in a nested loop.}, label={alg_nested_loop}]
  A two-layer loop
    loop out_begin, out_end, out_n
      some_operations()
      // Save the outer loop state before inner loop
      RegStore loop_regs,   addr_out_loop_reg
      RegStore offset_regs, addr_out_offset_reg
      loop in_begin, in_end, in_n
        some_operations()
    // Restore the outer loop state after the inner loop finishes
    RegLoad loop_regs,   addr_out_loop_reg
    RegLoad offset_regs, addr_out_offset_reg
\end{lstlisting}

\input{0604_loop_code_reduction.tex}

==> 0407_hw_motivation.tex <==
\subsection{Design Goals}

% find a minimalist but versatile hardware module that supports a analysis applicable to different user cases, which require multiple machine learning and deep learning models and unique analytic techniques.

We want to design a detection module that can give a yes-or-no answer for impostor detection without any subsequent processing on other devices. This greatly reduces the attack surface where the detection service itself can be attacked.

==> 0501_software.tex <==
\section{Models for Impostor Detection}
\label{sec_sw_model}

In this section, we present the models that can be used for impostor detection. We first present the accuracy of representative multi-class models, such as MLP and SVM, and the kernel ridge regression (KRR) model proposed as the most effective detection model. We then study the accuracy when using one-class models and show that it can be compensated with a statistical test.
%based on time series modeling.

\subsection{Dataset and Window Generation}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{./figures/180722_diffstep.eps}
    \caption{Detection accuracy when different window steps are used. A sampling step of 4 leads to a larger overlap between consecutive windows and has better classification accuracy of legitimate versus non-legitimate users.}
    \label{img_diffstep}
\end{figure*}

We test the accuracy of diffehrent ML/DL models for impostor detection on the smartphone-based recognition of human activities and postural transitions (HAPT) dataset~\cite{reyes2016transition} from UCI machine learning repository~\cite{Dua:2017}. The HAPT dataset contains the sensor readings from smartphone sensors. The smartphone is worn on the waist by a group of 30 participants of various ages from 19 to 48. The participants are asked to perform six kinds of activities including standing, sitting, walking, etc. and the transitions between them. The readings are collected in the meantime and later labeled with both the activity and user ID.

The HAPT dataset is initially designed to recognize human activities but we extend it to study the feasibility to distinguish users given that the activity is already recognized. We use the WALK subset in HAPT whose data has the same activity ID (WALK) to perform user classification. The raw inputs of each user are several long \textbf{sequences} of readings collected when the participants walked for several times. Each reading contains the 3-axial measurements of both the linear acceleration and angular velocity so it could be treated as a 6-element vector.

As some ML or DL models like MLP and SVM require an input of fixed size, we sample \textbf{windows} of the same length from the \textbf{sequences}. There are two considerations when we choose the window size. It is firstly desirable to recognize a user based on a window covering one or two full steps of a typical person. Also, we obtain the frequency domain information by doing FFT so choosing a power-of-2 window is a straightforward method. Hence, knowing that sensors are sampled at a rate of 50Hz, we choose a window size of 64 readings. 

However, consecutively sampling the windows with little-overlap can result in low recognition accuracy.~\gyreffig{img_diffstep} gives an intuitive heat-map of detection accuracy when the training and testing windows are sampled at a step of 4 readings and 32 readings. The model used is a single hidden layer MLP with 100 hidden neurons. Each block in the heat-map with a coordinate of (RID, TID) is the recognition accuracy when the model trained for the user labeled RID is used to recognize the testing data produced by the user labeled TID. As described by the color-bar, a darker block in the heat-map represents a lower recognition accuracy while a pure white block means all samples are classified correctly. The low-overlap sampling step of 32 is shown to generally have a worse accuracy. This is partly because a large step when collecting training windows can let the model only learn the features of a window which starts at the same phase within a step. If there is a misalignment between a testing window and windows in the training set with respect to the period of a step, a testing window is unlikely to be classified correctly.

To eliminate the problem, we produce fine-grained windows by using a smaller step when sampling the windows from the long sequences. The step is finally chosen to be 4 readings, which corresponds to an offset of 0.08s between consecutive windows and two consecutive windows have an overlap of 93.75\%.

We then need to separate the windows into a training set and a testing set. One thing to note here is that it is not reasonable to randomly pick windows from all the sequences. Due to the high overlap between consecutive windows from the same sequence, a random pick can result in high similarity between some training windows and testing windows, which makes the classification accuracy not representative. Instead, we claim that the windows in the training set and the testing set must be from different sequences. Therefore, the sequences are first labeled as training sequences or testing sequences and then the windows are divided according to the sequence they are from.


==> 0502_classification.tex <==
\subsection{Models Trained with Multi-class Data}

We investigate the ability of multi-class models trained to detect whether the current (test) user is not the correct user. We consider the case in real life when we have no knowledge of potential attackers. To emulate this situation, 25 out of the 30 users in the HAPT dataset are selected as registered users while the other 5 users act as unregistered users. For each registered user, models are trained using his/her data and some randomly picked sensor data of the other 24 registered users. In the training process, all the data from other 24 registered users are labeled as 'not being the correct user'. This is a method of labeling data in real application without losing the privacy of other registered users. The data of unregistered users is only used in testing to examine whether previously unseen attackers can be detected.

\begin{table}[ht]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{}                                                           & \multicolumn{6}{c|}{\textbf{All Users}}                                                             \\ \hline
\textbf{}                                                           & \textbf{TNR}   & \textbf{TPR}   & \textbf{Accuracy} & \textbf{R}    & \textbf{P}    & \textbf{F1}   \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Ridge\\ Regression\end{tabular}} & \textbf{80.77} & \textbf{66.05} & \textbf{73.41}    & \textbf{0.66} & \textbf{0.77} & \textbf{0.69} \\ \hline
\textbf{MLP-20}                                                     & \textbf{97.42} & \textbf{88.79} & \textbf{93.10}    & \textbf{0.89} & \textbf{0.96} & \textbf{0.91} \\ \hline
\textbf{MLP-50}                                                     & \textbf{98.31} & \textbf{92.70} & \textbf{95.51}    & \textbf{0.93} & \textbf{0.98} & \textbf{0.94} \\ \hline
\textbf{MLP-100}                                                    & \textbf{98.60} & \textbf{94.65} & \textbf{96.63}    & \textbf{0.95} & \textbf{0.98} & \textbf{0.96} \\ \hline
\textbf{MLP-200}                                                    & \textbf{98.41} & \textbf{95.72} & \textbf{97.06}    & \textbf{0.96} & \textbf{0.98} & \textbf{0.97} \\ \hline
\textbf{MLP-500}                                                    & \textbf{98.68} & \textbf{95.47} & \textbf{97.07}    & \textbf{0.95} & \textbf{0.99} & \textbf{0.96} \\ \hline
\textbf{MLP-50-25}                                                  & \textbf{98.13} & \textbf{94.49} & \textbf{96.31}    & \textbf{0.94} & \textbf{0.98} & \textbf{0.96} \\ \hline
\textbf{MLP-100-50}                                                 & \textbf{98.44} & \textbf{95.45} & \textbf{96.95}    & \textbf{0.95} & \textbf{0.98} & \textbf{0.96} \\ \hline
\textbf{MLP-200-100}                                                & \textbf{98.47} & \textbf{95.72} & \textbf{97.10}    & \textbf{0.96} & \textbf{0.98} & \textbf{0.97} \\ \hline
\textbf{SVM}                                                        & \textbf{99.26} & \textbf{97.57} & \textbf{98.42}    & \textbf{0.98} & \textbf{0.99} & \textbf{0.98} \\ \hline
\textbf{KRR}                                                        & \textbf{88.91} & \textbf{82.66} & \textbf{85.78}    & \textbf{0.83} & \textbf{0.87} & \textbf{0.83} \\ \hline
\end{tabular}
}
\caption{Recognition accuracy of binary classification models}
\label{tbl_accuracy_binary}
\end{table}

We present the accuracy of binary classification models in~\gyreftbl{tbl_accuracy_binary} where each row corresponds to one model. The results shows that SVM performs best for all the metrics. Among the single-layer MLP models, the single hidden layer with 500 hidden neurons has the best average accuracy and increasing the number of hidden layers can slightly improve the average accuracy. The KRR method requiring manual feature extraction performs much better than the ridge regression model on raw data but has a lower accuracy than MLP and SVM based models.



\iffalse
\bheading{Regression}


\bheading{Multilayer Perceptron}


\bheading{Support Vector Machine}
\fi


==> 0503_oneclass.tex <==
\subsection{One-class Models for Impostor Detection}

While the previous models for classification always need other users' data for training, it is desirable for a user to have a one-class model trained with only his/her own data. %From the application perspective, privacy concerns are raised when 
To train multi-class models, the detection provider needs users' consent to use their data to train the models for other people. This requirement raises privacy concerns for users and has a high probability to be rejected. The one-class models can avoid asking for the data of other users. 
From the security perspective, the training with data from certain users can be unreliable. It is non-trivial to predict how an unregistered anomalous user will differ from registered users. It is hence hard to guarantee that a multi-class model can learn all the patterns of anomalous users using only registered users' data in the training. 

We test two one-class models, the one-class SVM and a LSTM-based model for time-series modeling. The one-class SVM has an average accuracy of 69.22\% which is about thirty percent worse than the best multi-class models. The LSTM-based model makes predictions for every sensor reading in the sample window. The classification result is given by comparing the average prediction error with a threshold obtain from the training set. The LSTM-based models have an accuracy about 70 percent for both real user and wrong users, which is similar to the one-class SVM model. It is also found that the accuracy doesn't improve much when the number of hidden nodes is increased.
%Moreover, the worst recognized user by one-class SVM encounters an accuracy of 17.43\%. This worst-case accuracy will prevent any user from adopting this model for protection.The LSTM-based model having 500 hidden nodes can achieve an accuracy of more than ninety percent, which is comparable to the multi-class models. However, the LSTM-based model also performs badly by recognizing the user 19 with an accuracy about fifty percent.

%From the system design perspective, the one-class models can benefit from local incremental training with the data produced by the real user. This will alleviate the reliability on the communication of remote servers and at the same time reduce the attack vectors to the round trip for remote processing.

\begin{table}[ht]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{}                                                             & \multicolumn{6}{c|}{\textbf{All Users}}                                                             \\ \hline
\textbf{}                                                             & \textbf{TNR}   & \textbf{TPR}   & \textbf{Accuracy} & \textbf{R}    & \textbf{P}    & \textbf{F1}   \\ \hline
\textbf{OCSVM}                                                        & \textbf{64.24} & \textbf{74.19} & \textbf{69.22}    & \textbf{0.74} & \textbf{0.59} & \textbf{0.65} \\ \hline
\textbf{LSTM-20}                                                      & \textbf{70.53} & \textbf{64.96} & \textbf{67.75}    & \textbf{0.65} & \textbf{0.54} & \textbf{0.57} \\ \hline
\textbf{LSTM-50}                                                      & \textbf{72.43} & \textbf{67.04} & \textbf{69.74}    & \textbf{0.67} & \textbf{0.57} & \textbf{0.60} \\ \hline
\textbf{LSTM-100}                                                     & \textbf{72.20} & \textbf{69.27} & \textbf{70.73}    & \textbf{0.69} & \textbf{0.58} & \textbf{0.62} \\ \hline
\textbf{LSTM-200}                                                     & \textbf{67.88} & \textbf{71.60} & \textbf{69.74}    & \textbf{0.72} & \textbf{0.58} & \textbf{0.62} \\ \hline
\textbf{LSTM-500}                                                     & \textbf{67.57} & \textbf{74.42} & \textbf{70.99}    & \textbf{0.74} & \textbf{0.60} & \textbf{0.65} \\ \hline \hline
\textbf{\begin{tabular}[c]{@{}l@{}}LSTM-200-\\ KS-OCSVM\end{tabular}} & \textbf{74.82} & \textbf{92.25} & \textbf{83.53}    & \textbf{0.92} & \textbf{0.80} & \textbf{0.84} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}LSTM-200-\\ KS-Vote\end{tabular}}  & \textbf{94.62} & \textbf{83.31} & \textbf{88.97}    & \textbf{0.83} & \textbf{0.91} & \textbf{0.83} \\ \hline
\end{tabular}
}
\caption{Recognition accuracy of one-class models}
\label{tbl_accuracy_oneclass}
\end{table}

%\bheading{One class SVM}

%\bheading{LSTM}


\iffalse
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real\\ User ID\end{tabular}}} & \multicolumn{3}{c|}{OC-SVM}                                                         \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                                                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} \\ \hline
1                                                                                             & 53.58                    & 0                        & 3                             \\ \hline
2                                                                                             & 96.65                    & 22.22                    & 2                             \\ \hline
3                                                                                             & 97                       & 30.91                    & 18                            \\ \hline
4                                                                                             & 98.6                     & 58.85                    & 4                             \\ \hline
5                                                                                             & 86.31                    & 0                        & 4                             \\ \hline
6                                                                                             & 72.83                    & 0                        & 4                             \\ \hline
7                                                                                             & 50.16                    & 0                        & 3                             \\ \hline
8                                                                                             & 29.55                    & 0                        & 3                             \\ \hline
9                                                                                             & 83.54                    & 0                        & 16                            \\ \hline
10                                                                                            & 65.4                     & 0                        & 4                             \\ \hline
11                                                                                            & 96.79                    & 40.08                    & 11                            \\ \hline
12                                                                                            & 86.07                    & 9.19                     & 25                            \\ \hline
13                                                                                            & 45.75                    & 0                        & 3                             \\ \hline
14                                                                                            & 95.62                    & 1.36                     & 18                            \\ \hline
15                                                                                            & 88.54                    & 0                        & 4                             \\ \hline
16                                                                                            & 98.28                    & 70.45                    & 18                            \\ \hline
17                                                                                            & 84.34                    & 0                        & 18                            \\ \hline
18                                                                                            & 98.93                    & 71.36                    & 18                            \\ \hline
19                                                                                            & 17.43                    & 0                        & 1                             \\ \hline
20                                                                                            & 25.66                    & 0                        & 1                             \\ \hline
21                                                                                            & 84.1                     & 0                        & 3                             \\ \hline
22                                                                                            & 49.66                    & 0                        & 3                             \\ \hline
23                                                                                            & 45.37                    & 0                        & 3                             \\ \hline
24                                                                                            & 98.45                    & 60.85                    & 24                            \\ \hline
25                                                                                            & 97.91                    & 40.28                    & 25                            \\ \hline
Avg                                                                                           & 68.39                    & 15.02                    &                               \\ \hline
\end{tabular}
\end{table}

\fi

==> 0504_frequency.tex <==
\subsection{Introduction of Frequency Information}

Previous work~\cite{lee2017implicit} used statistical methods to find the most valuable features in both time and frequency domains and demonstrated an improvement on recognition accuracy. %We focus more on the DL models and 
We study if the frequency domain information can be introduced to improve the accuracy of one-class models %evaluate the impact on classification accuracy when the frequency domain information is added. The additional input to the DL models is the frequency components which 
The frequency domain features can be computed through a discrete Fourier transform (DFT) as~\gyrefeq{eq_freq_amp}. The complex frequency components are presented as two arrays of numbers which account for the real part and the imaginary part respectively. The squared amplitudes of all the frequency components could be computed by our processing module and used as additional feature afterwards. Different from~\cite{lee2017implicit} which further manually extracts the frequency domain features such as the most significant components, we expect the DL models can automatically learn useful features from the frequency domain amplitudes.



\bheading{Binary Classification Models} We compare the accuracy to recognize a given window using only time domain features and using both time and frequency domain features. The time domain features are the sums of the squared amplitudes of accelerometer and gyroscope readings as expressed in~\gyrefeq{eq_time_amp}. In a 64-point window, we could get 64 amplitude features from the accelerometer and another 64 features from the gyroscope.
\begin{equation}
\label{eq_time_amp}
\begin{split}
acc_{amp}[i]& = acc_x[i]^2 + acc_y[i]^2 + acc_z[i]^2 \\
gyr_{amp}[i]& = gyr_x[i]^2 + gyr_y[i]^2 + gyr_z[i]^2 \\
&i = 0, 1,..., window\_len-1
\end{split}
\end{equation}
The frequency features are the amplitudes of frequency components of the current window.~\gyrefeq{eq_freq_amp} describes how the features are obtained. $e^{\frac{-i2\pi kj}{window\_len}}$ terms are constants that can be computed before the inference. $acc/gyr_f[k]$ are complex numbers produced by the DFT procedure. We only captures their amplitude information by computing their norms.

There are originally 64 such features from both the accelerometer and the gyroscope for a 64-point window. However, since ${acc/gyr}_{amp}[j]$ are all real numbers, ${acc/gyr}_{f}[k], k = 1,...,31$ can be proved~\cite{wiki:dft} to be the complex conjugate of $acc/gyr_{f}[64-k]$ and their norms are the same. Therefore, only the first half of $acc/gyr_{famp}[k], k = 0,1,...,32$ (33 components in total for each sensor) needs to be saved as input features.
\begin{equation}
\label{eq_freq_amp}
\begin{split}
acc_{f}[k]   & = \textstyle \sum_{j=0}^{window\_len-1} acc_{amp}[j] \times e^{\frac{-i2\pi kj}{window\_len}} \\
&(e^{\frac{-i2\pi kj}{window\_len}} = \cos \tfrac{-2\pi kj}{window\_len} + i \sin \tfrac{-2\pi kj}{window\_len}) \\
acc_{ampf}[k]& = \norm{acc_{f}[k]} = \textstyle \sqrt{Re(acc_{f}[k])^2 + Im(acc_{f}[k])^2} \\
gyr_{f}[k]   & = \textstyle \sum_{j=0}^{window\_len-1} gyr_{amp}[j] \times e^{\frac{-i2\pi kj}{window\_len}} \\
gyr_{ampf}[k]& = \norm{gyr_{f}[k]} = \textstyle \sqrt{Re(gyr_{f}[k])^2 + Im(gyr_{f}[k])^2} \\
&k = 0,1,..., window\_len-1
\end{split}
\end{equation}
\gyreftbl{tbl_freq_binary} shows the impact of adding frequency-domain features on the recognition accuracy. The features increase the best average accuracy of LR, MLP and SVM models by 21.17\%, 3.78\% and 4.90\% respectively. A more significant improvement can be found for the users having minimum recognition accuracy. The accuracy of the worst recognized user is increased by 30.03\%, 6.63\% and 14.71\% for the three models. 
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
Model                                                      & Avg   & Min   & Min User & Model                                                          & Avg   & Min   & Min User \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ LR\end{tabular}          & 66.4  & 46.52 & 6        & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ LR\end{tabular}          & 87.57 & 76.55 & 10       \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-10\end{tabular}      & 75.15 & 50.9  & 6        & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-10\end{tabular}      & 91.52 & 79.69 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-20\end{tabular}      & 79.56 & 60.28 & 13       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-20\end{tabular}      & 92.4  & 81.47 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-50\end{tabular}      & 84.07 & 61.79 & 13       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-50\end{tabular}      & 93.16 & 82.21 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-100\end{tabular}     & 86.89 & 68.54 & 13       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-100\end{tabular}     & 93.29 & 83.04 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-200\end{tabular}     & 87.87 & 66.67 & 6        & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-200\end{tabular}     & 93.16 & 82    & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-500\end{tabular}     & 88.45 & 69.31 & 13       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-500\end{tabular}     & 92.92 & 80.84 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-1000\end{tabular}    & 87.99 & 71.07 & 1        & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-1000\end{tabular}    & 92.25 & 80.25 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-50-25\end{tabular}   & 86.5  & 66.3  & 5        & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-50-25\end{tabular}   & 94.1  & 85.96 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-100-50\end{tabular}  & 89.3  & 72.3  & 13       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-100-50\end{tabular}  & 94.38 & 84.17 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ MLP-200-100\end{tabular} & 90.6  & 79.33 & 6        & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ MLP-200-100\end{tabular} & 94.37 & 85.54 & 1        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ SVM\end{tabular}         & 90.44 & 71.5  & 5        & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ SVM\end{tabular}         & 95.34 & 86.21 & 5        \\ \hline
\end{tabular}
}
\caption{Improving binary classification models with frequency-domain features}
\label{tbl_freq_binary}
\end{table}


\bheading{One-class models}
We study whether frequency-domain information will improve the accuracy of one-class models. The one-class models using only time-domain amplitude features in the left part of~\gyreftbl{tbl_freq_oc} have low average recognition accuracy for all the users. Moreover, for the user being worst recognized, the accuracy stays around 10 percent even if the size of LSTM model is increased. Hence one-class models using only time-domain features are not acceptable security solutions to protect the smartphone.

On the other hand, including frequency-domain features obtained is shown to make one-class models usable. For the one-class SVM (OCSVM) model, we include the frequency features of a window which is computed according to~\gyrefeq{eq_freq_amp}. The frequency domain information increases the OCSVM model's average accuracy by 29.81\% and worst-case accuracy from 7.42\% to 53.65\%. While the worst-case accuracy of OCSVM is still not satisfactory for user 6, the LSTM-based DL model benefits more from the extra frequency features. For the LSTM-based model, we regenerate the data so that each reading contains not only the amplitude features but also the 64-point DFT result of the latest 64 readings. As shown in the right part of~\gyreftbl{tbl_freq_oc}, the average accuracy of LSTM-based model can be increased to 94.25\%. Even in the worst case, the user can still be protected with an accuracy of more than 80 percent.
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
Model                                                   & Avg   & Min   & Min User & Model                                                       & Avg   & Min   & Min User \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ OCSVM\end{tabular}    & 55.87 & 7.42  & 19       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ OCSVM\end{tabular}    & 85.68 & 53.65 & 6        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ LSTM-10\end{tabular}  & 61.67 & 4.28  & 19       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ LSTM-10\end{tabular}  & 65.68 & 12.36 & 19       \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ LSTM-20\end{tabular}  & 61.08 & 4.58  & 19       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ LSTM-20\end{tabular}  & 70.63 & 18.96 & 19       \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ LSTM-50\end{tabular}  & 61.58 & 7.61  & 20       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ LSTM-50\end{tabular}  & 77.63 & 28.62 & 23       \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ LSTM-100\end{tabular} & 67.52 & 10.59 & 19       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ LSTM-100\end{tabular} & 86.54 & 52.34 & 1        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ LSTM-200\end{tabular} & 67.74 & 8.4   & 19       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ LSTM-200\end{tabular} & 94.25 & 80.25 & 7        \\ \hline
\begin{tabular}[c]{@{}l@{}}Amp-\\ LSTM-500\end{tabular} & 68.35 & 7.45  & 19       & \begin{tabular}[c]{@{}l@{}}Amp-FFT-\\ LSTM-500\end{tabular} & 92.96 & 80.49 & 7        \\ \hline
\end{tabular}
}
\caption{Improving one-class models with frequency-domain features}
\label{tbl_freq_oc}
\end{table}

==> 0505_kstest.tex <==
\subsection{Enhance one-class models with KS Test}
\label{sec_ks_test}

~\gyreftbl{tbl_accuracy_oneclass} indicates that characterizing the user behaviors with the average of sensor prediction errors is not enough. We opt to assume that normal sensor samples can feature one of several reference patterns of the real user. To be more specific, a sample is considered to be from a certain user if the distribution of its sensor prediction errors is similar to at least one such distribution in that user's training set.

%We study whether statistics test can be included to make the classification more robust. 

We measure the difference between two error distributions with Kolmogorov-Smirnov test (KS test). KS test finds the maximum difference (also termed KS-test-statistic) between two empirical distribution function, $F_1(x)$ and $F_2(x)$, as shown in~\gyrefeq{eq_kstest_d}. 

\begin{equation}
\centering
  D(F_1, F_2) = \sup_x \norm{F_1(x) - F_2(x)}
\label{eq_kstest_d}
\end{equation}

We classify a testing sample by doing a majority vote using the KS-test-statistic. We first randomly choose 20 samples of prediction errors from the training set and use them to represent the reference distributions. In the testing phase, the error distribution of each testing sample is compared to all the reference distributions. If half of the KS-test-statistic's are larger than a commonly used threshold, the current sample is considered from an attacker. This method corresponds to the row of \textbf{LSTM-200-KS-Vote} in~\gyreftbl{tbl_accuracy_oneclass} and gives an average accuracy of 88.97\%, which gets much closer to the accuracy of multi-class models. This voting-based method achieves a high TNR of 94.62\% but a lower TPR of 83.31\%, which means it is a loose model providing good usability for the real user but limited security against impostors.

We also characterize the cluster of reference distributions and then recognize outliers as attackers. A one-class SVM model is applied on top of the KS-test-statistic's. While still using 20 reference samples, we now represent each sample as $(D_1, D_2,..., D_{20})$, which are its KS-test-statistic's with 20 reference samples. We train a one-class SVM model using the features of training samples. The features of testing sample are fed into the one-class SVM model to obtain a binary classification result. This method corresponds to the row of \textbf{LSTM-200-KS-OCSVM} in~\gyreftbl{tbl_accuracy_oneclass} and gives an average accuracy of 83.53\%. Using one-class SVM achieves a high TPR of 92.25\% but a lower TPR of 74.82\%, which means it is a strict model providing good security against impostors but can erroneously reject the real user.

==> 0601_security_analysis.tex <==
\subsection{Security against Unregistered Impostors}
\label{sec_security_analysis}

\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{}                                                             & \textbf{TPR(Registered)} & \textbf{TPR(Unregistered)} & \textbf{TPR Difference} \\ \hline
\textbf{MLP-50}                                                       & \textbf{92.41}           & \textbf{94.09}             & \textbf{1.68}           \\ \hline
\textbf{MLP-500}                                                      & \textbf{95.64}           & \textbf{94.65}             & \textbf{-0.99}          \\ \hline
\textbf{MLP-50-25}                                                    & \textbf{91.00}           & \textbf{92.52}             & \textbf{1.53}           \\ \hline
\textbf{MLP-200-100}                                                  & \textbf{92.84}           & \textbf{93.62}             & \textbf{0.78}           \\ \hline
\textbf{SVM}                                                          & \textbf{97.53}           & \textbf{97.73}             & \textbf{0.20}           \\ \hline
\textbf{KRR}                                                          & \textbf{82.60}           & \textbf{82.92}             & \textbf{0.32}           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}LSTM-200-\\ KS-OCSVM\end{tabular}} & \textbf{92.21}           & \textbf{92.43}             & \textbf{0.22}           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}LSTM-200-\\ KS-Vote\end{tabular}}  & \textbf{83.39}           & \textbf{82.94}             & \textbf{-0.45}          \\ \hline
\end{tabular}
}
\caption{Recognition accuracy of registered and unregistered users}
\label{tbl_reg_unreg}
\end{table}

We verify the applicability of models when potential impostors are likely to be unregistered users. For each registered user, the other 24 registered users are used as impostors whose data are available in the training dataset. The 5 users whose data is not used during training are considered unforeseen impostor. 

We compare the average accuracy to recognize registered users and unregistered users in~\gyreftbl{tbl_reg_unreg}. The accuracy is the TPR in these experiments as it is evaluated only on other users' data. The result shows that the models trained with only registered users' data can detect unregistered users at a similar accuracy. The difference of TPR between registered users and unregistered users given in the last column show that most models can even detect unregistered users slightly more accurately than registered users.

\iffalse
\begin{table*}[h!]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{}                                                             & \multicolumn{1}{c|}{\textbf{Real User}} & \multicolumn{5}{l|}{\textbf{Other Registered Users}}                               & \multicolumn{5}{l|}{\textbf{Unregistered Users}}                                   \\ \hline
\textbf{}                                                             & \textbf{TNR}                            & \textbf{TPR}   & \textbf{Accuracy} & \textbf{R}    & \textbf{P}    & \textbf{F1}   & \textbf{TPR}   & \textbf{Accuracy} & \textbf{R}    & \textbf{P}    & \textbf{F1}   \\ \hline
\textbf{MLP-50}                                                       & \textbf{98.31}                          & \textbf{92.41} & \textbf{95.36}    & \textbf{0.92} & \textbf{0.98} & \textbf{0.94} & \textbf{94.09} & \textbf{96.20}    & \textbf{0.94} & \textbf{0.98} & \textbf{0.95} \\ \hline
\textbf{MLP-500}                                                      & \textbf{98.68}                          & \textbf{95.64} & \textbf{97.16}    & \textbf{0.96} & \textbf{0.99} & \textbf{0.97} & \textbf{94.65} & \textbf{96.66}    & \textbf{0.95} & \textbf{0.99} & \textbf{0.96} \\ \hline
\textbf{MLP-50-25}                                                    & \textbf{96.05}                          & \textbf{91.00} & \textbf{93.52}    & \textbf{0.91} & \textbf{0.95} & \textbf{0.92} & \textbf{92.52} & \textbf{94.29}    & \textbf{0.93} & \textbf{0.96} & \textbf{0.94} \\ \hline
\textbf{MLP-200-100}                                                  & \textbf{97.90}                          & \textbf{92.84} & \textbf{95.37}    & \textbf{0.93} & \textbf{0.98} & \textbf{0.94} & \textbf{93.62} & \textbf{95.76}    & \textbf{0.94} & \textbf{0.98} & \textbf{0.95} \\ \hline
\textbf{SVM}                                                          & \textbf{99.26}                          & \textbf{97.53} & \textbf{98.40}    & \textbf{0.98} & \textbf{0.99} & \textbf{0.98} & \textbf{97.73} & \textbf{98.50}    & \textbf{0.98} & \textbf{0.99} & \textbf{0.98} \\ \hline
\textbf{KRR}                                                          & \textbf{88.91}                          & \textbf{82.60} & \textbf{85.75}    & \textbf{0.83} & \textbf{0.87} & \textbf{0.83} & \textbf{82.92} & \textbf{85.91}    & \textbf{0.83} & \textbf{0.87} & \textbf{0.83} \\ \hline \hline
\textbf{\begin{tabular}[c]{@{}l@{}}LSTM-200-\\ KS-OCSVM\end{tabular}} & \textbf{74.82}                          & \textbf{92.21} & \textbf{83.51}    & \textbf{0.92} & \textbf{0.80} & \textbf{0.84} & \textbf{92.43} & \textbf{83.63}    & \textbf{0.92} & \textbf{0.81} & \textbf{0.84} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}LSTM-200-\\ KS-Vote\end{tabular}}  & \textbf{94.62}                          & \textbf{83.39} & \textbf{89.00}    & \textbf{0.83} & \textbf{0.92} & \textbf{0.83} & \textbf{82.94} & \textbf{88.78}    & \textbf{0.83} & \textbf{0.88} & \textbf{0.83} \\ \hline
\end{tabular}
\caption{Recognition accuracy of registered and unregistered users}
\label{tbl_reg_unreg}
\end{table*}
\fi

==> 06022_combined_metric.tex <==
\subsection{Combined Metrics}
\label{sec_combined_metrics}

In this section, we propose to use a single metric for users to choose their models for detection with the tradeoff between accuracy, performance and memory usage. In most use cases, users don't need to be aware of the details of the model that can be applied but they can specify the key factor they care about. For instance, some users may want to get the highest accuracy without caring about the memory usage or performance. Some other users may want to save the memory usage while maintain a reasonable accuracy. 

We provide a generalized decision method in~\gyrefeq{eq_combined_metric} to consider all the metrics. Each model in a certain scope has a penalty for a higher error rate, a longer execution time or a larger memory usage. To make fair comparison, we identify the minimum error rate, the minimum execution time and the minimal memory usage in the set of available models. The penalty in each dimension is normalized to its corresponding minimum in the model set. The combined metric is computed as a weighted sum of three normalize penalties. The weights can be controlled by the user based on the user's preference.
\begin{equation}
\begin{split}
    %for i such that & ErrRate_i = Accuracy_i > thErr \\
    %                & and Perf_i > thPerf \\
    &Score(Model_i) = \\
    &\frac{2}{\begin{split}
                            &a1 \times NormFNR_i + 
                             a2 \times NormFPR_i + \\
                            &b1 \times NormTime_i + 
                              b2 \times NormMem_i\end{split}}
                              \\
                              \\
    &(a1 + a2 + b1 + b2 = 2) \\
                    %& w_a \times NormErrRate_i \\
                   %+ & w_t \times NormTime_i \\
                   %+ & w_m \times NormMemUsage_i \\
    % (if~ErrRate_i = & 1-Accuracy_i > thErrRate \\
    %             and~& ~Time_i > thTime) \\
    %     ErrRate_i = & 1 - Accuracy_i \\
    % NormErrRate_i = & \frac{ErrRate_i}{Min(ErrRate)} \\
        &~NormFNR_i =  \frac{FNR_i}{Min(FNR)} \\
        &~NormFPR_i =  \frac{FNR_i}{Min(FPR)} \\
        &NormTime_i =  \frac{Time_i}{Min(Time)} \\
        &~NormMem_i =  \frac{MemUsage_i}{Min(MemUsage)}
\end{split}
    %NormErrRate_i = \frac{ErrRate_i}{MinErrRate} \\
    %NormPerf_i = \frac{Perf_i}{MinPerf} \\
    %NormMemUsage_i = \frac{MemUsage_i}{MinMemUsage} \\
    %ErrRate_i = Accuracy_i > thErr \\
    %Perf_i > thPerf \\
\label{eq_combined_metric}
\end{equation}


\begin{table*}[h]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Weights\\ (a1,a2,b1,b2)\end{tabular}}                                    & \multicolumn{1}{c|}{Model Name} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Normalized\\ FNR\\ (security)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Normalized\\ FPR\\ (usability)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Normalized\\ Execution\\ Time\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Normalized\\ Memory\\ Usage\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Combined\\ Metric\end{tabular}} \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}(0.5, 0.5, 0.5, 0.5)\\ Equal weights\end{tabular}}                            & MLP-50                          & 3.00                                                                                       & 2.29                                                                                        & 1.00                                                                                       & 1.00                                                                                     & 0.55                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-500                         & 1.86                                                                                       & 1.80                                                                                        & 9.98                                                                                       & 10.00                                                                                    & 0.17                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-50-25                       & 3.59                                                                                       & 5.38                                                                                        & 1.07                                                                                       & 1.07                                                                                     & 0.36                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-200-100                     & 2.89                                                                                       & 2.86                                                                                        & 5.03                                                                                       & 5.04                                                                                     & 0.25                                                                           \\ \cline{2-7} 
                                                                                                                         & SVM                             & 1.00                                                                                       & 1.00                                                                                        & 37.05                                                                                      & 17.34                                                                                    & 0.07                                                                           \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}(0.9, 0.1, 0.5, 0.5)\\ FNR critical\end{tabular}}                             & MLP-50                          & 3.00                                                                                       & 2.29                                                                                        & 1.00                                                                                       & 1.00                                                                                     & 0.51                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-500                         & 1.86                                                                                       & 1.80                                                                                        & 9.98                                                                                       & 10.00                                                                                    & 0.17                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-50-25                       & 3.59                                                                                       & 5.38                                                                                        & 1.07                                                                                       & 1.07                                                                                     & 0.41                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-200-100                     & 2.89                                                                                       & 2.86                                                                                        & 5.03                                                                                       & 5.04                                                                                     & 0.25                                                                           \\ \cline{2-7} 
                                                                                                                         & SVM                             & 1.00                                                                                       & 1.00                                                                                        & 37.05                                                                                      & 17.34                                                                                    & 0.07                                                                           \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}(0.9, 0.1, 0.9, 0.1)\\ FNR critical\\ Execution time\\ critical\end{tabular}} & MLP-50                          & 3.00                                                                                       & 2.29                                                                                        & 1.00                                                                                       & 1.00                                                                                     & 0.51                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-500                         & 1.86                                                                                       & 1.80                                                                                        & 9.98                                                                                       & 10.00                                                                                    & 0.17                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-50-25                       & 3.59                                                                                       & 5.38                                                                                        & 1.07                                                                                       & 1.07                                                                                     & 0.41                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-200-100                     & 2.89                                                                                       & 2.86                                                                                        & 5.03                                                                                       & 5.04                                                                                     & 0.25                                                                           \\ \cline{2-7} 
                                                                                                                         & SVM                             & 1.00                                                                                       & 1.00                                                                                        & 37.05                                                                                      & 17.34                                                                                    & 0.06                                                                           \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}(0.1, 0.9, 0.5, 0.5)\\ FPR critical\end{tabular}}                             & MLP-50                          & 3.00                                                                                       & 2.29                                                                                        & 1.00                                                                                       & 1.00                                                                                     & 0.59                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-500                         & 1.86                                                                                       & 1.80                                                                                        & 9.98                                                                                       & 10.00                                                                                    & 0.17                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-50-25                       & 3.59                                                                                       & 5.38                                                                                        & 1.07                                                                                       & 1.07                                                                                     & 0.32                                                                           \\ \cline{2-7} 
                                                                                                                         & MLP-200-100                     & 2.89                                                                                       & 2.86                                                                                        & 5.03                                                                                       & 5.04                                                                                     & 0.25                                                                           \\ \cline{2-7} 
                                                                                                                         & SVM                             & 1.00                                                                                       & 1.00                                                                                        & 37.05                                                                                      & 17.34                                                                                    & 0.07                                                                           \\ \hline
\end{tabular}
\caption{The combined metric of models used in scenario 2 when users care most about different factors.}
\label{tbl_combined_metric_2}
\end{table*}

\begin{table*}[h]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Weights\\ (a1,a2,b1,b2)\end{tabular}}                                    & \multicolumn{1}{c|}{Model Name} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Normalized\\ FNR\\ (security)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Normalized\\ FPR\\ (usability)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Normalized\\ Execution\\ Time\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Normalized\\ Memory\\ Usage\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Combined\\ Metric\end{tabular}} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}(0.5, 0.5, 0.5, 0.5)\\ Equal weights\end{tabular}}                            & OCSVM                           & 3.06                                                                                       & 6.03                                                                                        & 1.00                                                                                       & 1.00                                                                                     & 0.36                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-th                     & 3.37                                                                                       & 5.54                                                                                        & 1.32                                                                                       & 2.78                                                                                     & 0.31                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-KS-OCSVM               & 1.00                                                                                       & 4.36                                                                                        & 1.87                                                                                       & 2.82                                                                                     & 0.40                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-KS-Vote                & 1.98                                                                                       & 1.00                                                                                        & 1.84                                                                                       & 2.81                                                                                     & 0.52                                                                           \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}(0.9, 0.1, 0.5, 0.5)\\ FNR critical\end{tabular}}                             & OCSVM                           & 3.06                                                                                       & 6.03                                                                                        & 1.00                                                                                       & 1.00                                                                                     & 0.46                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-th                     & 3.37                                                                                       & 5.54                                                                                        & 1.32                                                                                       & 2.78                                                                                     & 0.35                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-KS-OCSVM               & 1.00                                                                                       & 4.36                                                                                        & 1.87                                                                                       & 2.82                                                                                     & 0.54                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-KS-Vote                & 1.98                                                                                       & 1.00                                                                                        & 1.84                                                                                       & 2.81                                                                                     & 0.48                                                                           \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}(0.9, 0.1, 0.9, 0.1)\\ FNR critical\\ Execution time\\ critical\end{tabular}} & OCSVM                           & 3.06                                                                                       & 6.03                                                                                        & 1.00                                                                                       & 1.00                                                                                     & 0.46                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-th                     & 3.37                                                                                       & 5.54                                                                                        & 1.32                                                                                       & 2.78                                                                                     & 0.40                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-KS-OCSVM               & 1.00                                                                                       & 4.36                                                                                        & 1.87                                                                                       & 2.82                                                                                     & 0.61                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-KS-Vote                & 1.98                                                                                       & 1.00                                                                                        & 1.84                                                                                       & 2.81                                                                                     & 0.52                                                                           \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}(0.1, 0.9, 0.5, 0.5)\\ FPR critical\end{tabular}}                             & OCSVM                           & 3.06                                                                                       & 6.03                                                                                        & 1.00                                                                                       & 1.00                                                                                     & 0.30                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-th                     & 3.37                                                                                       & 5.54                                                                                        & 1.32                                                                                       & 2.78                                                                                     & 0.27                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-KS-OCSVM               & 1.00                                                                                       & 4.36                                                                                        & 1.87                                                                                       & 2.82                                                                                     & 0.31                                                                           \\ \cline{2-7} 
                                                                                                                         & LSTM-200-KS-Vote                & 1.98                                                                                       & 1.00                                                                                        & 1.84                                                                                       & 2.81                                                                                     & 0.58                                                                           \\ \hline
\end{tabular}
\caption{The combined metric of models used in scenario 2 when users care most about different factors.}
\label{tbl_combined_metric_2}
\end{table*}

\iffalse
\gyreffig{img_pnlty1} shows the penalties when the user cares most about the accuracy and uses $(w_a, w_t, w_m) = (0.9, 0.05, 0.05)$ as the weights. In this case, the basic LSTM model which suffers from the the low accuracy of 71.60\% has the highest penalty. The LSTM models with KS support improves the accuracy but has more penalties than the multi-class models. The multi-class models all have small penalties as their accuracy is larger than 90\%.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{./figures/pnlty1.pdf}
    \caption{The combined penalty emphasizing the accuracy}
    \label{img_pnlty1}
\end{figure}

\gyreffig{img_pnlty2} shows a different user preference when the memory storage is the critical factor. A weight vector as $(w_a, w_t, w_m) = (0.05, 0.05, 0.9)$ is used. The result shows that the SVM model, even though having the highest detection accuracy, becomes the least preferred model due to its large model size. The small MLP models like MLP-50 and MLP-50-25 are shown to be the best choices as they use much less memory but stall achieve a high accuracy.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{./figures/pnlty2.pdf}
    \caption{The combined penalty emphasizing the memory usage}
    \label{img_pnlty2}
\end{figure}
\fi

==> 0604_loop_code_reduction.tex <==
%\subsection{Program Code Size}

\gyreftbl{tbl_code_size} shows the code size to run algorithms, which provide best detection accuracy in both scenarios, in the \modulename module. Note that the two complex models, \textbf{LSTM-200-KS-OCSVM} and \textbf{LSTM-200-KS-Vote}, in Scenario 2 both consist of three stages. Specifically, \textbf{LSTM-200-KS-OCSVM}~can be divided into \textbf{LSTM-200}, \textbf{KS-40} and \textbf{OCSVM (after KS-40)} and \textbf{LSTM-200-KS-Vote} can be divided into \textbf{LSTM-200}, \textbf{KS-40} and \textbf{Vote-KS}. These stages benefit differently from the nested loop support so we discuss the stages separately in \gyreftbl{tbl_code_size}.

The sizes of MLP models used in Scenario 1 grow with the model size. This is because we divide a matrix into multiple blocks when it is too big to put all the output nodes in the local scratchpad.

The loop support shows a 182.2X and 33.7X reduction in code size for SVM and OCSVM models which have the biggest code size when the loop support is not implemented. %Actually, the flexibility of instruction encoding makes it possible to encode any (OC)SVM model using a Gaussian kernel with 432 bytes (27 instructions) so that 
The small OCSVM model in~\textbf{LSTM-200-KS-OCSVM} also benefits from the loop support to reduce the code size by 5.5X. The KS test has two outer loops for each prediction error and each reference distribution so the nested loop support can also be applied and this reduces the code size by 147.7X. The small code size shows that with the loop support, it is feasible to put the code in a dedicated memory for fast access.%, which satisfies the design goal to~\textbf{reduce the code size for fast initialization} as mentioned in~\gyrefsec{sec_detection_energy}.

\begin{table}[h]
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{|c|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{}     &                           & SIDE  & SIDE+ & \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Scenario\\ 1\end{tabular}} & MLP-50                                                            & 112                                                                             & N/A                                                                            & N/A                                                            \\ \cline{2-5} 
                                                                      & MLP-500                                                           & 224                                                                             & N/A                                                                            & N/A                                                            \\ \cline{2-5} 
                                                                      & MLP-50-25%\begin{tabular}[c]{@{}l@{}}MLP-\\ 50-25\end{tabular}              
                                                                      & 208                                                                             & N/A                                                                            & N/A                                                            \\ \cline{2-5} 
                                                                      & MLP-200-100%\begin{tabular}[c]{@{}l@{}}MLP-\\ 200-100\end{tabular}            
                                                                      & 224                                                                             & N/A                                                                            & N/A                                                            \\ \cline{2-5} 
                                                                      & SVM                                                               & 78.7k                                                                           & 432                                                                            & 182.2X                                                         \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Scenario\\ 2\end{tabular}} & OCSVM                                                             & 14,6k                                                                           & 432                                                                            & 33.7X                                                          \\ \cline{2-5} 
                                                                      & LSTM-200                                                          & 560                                                                             & N/A                                                                            & N/A                                                            \\ \cline{2-5} 
                                                                      & KS-40 (20 Refs) %\begin{tabular}[c]{@{}l@{}}KS-40\\ (20 Refs)\end{tabular}      
                                                                      & 52k %\begin{tabular}[c]{@{}l@{}}2,6k*20\\ =52k\end{tabular}                          
                                                                      & 352                                                                            & 147.7X                                                         \\ \cline{2-5} 
                                                                      & OCSVM-KS %\begin{tabular}[c]{@{}l@{}}OCSVM\\ (after KS\\ test)\end{tabular} 
                                                                      & 2.4k                                                                            & 432                                                                            & 5.5X                                                           \\ \cline{2-5} 
                                                                      & Vote-KS                                                           & 32                                                                              & N/A                                                                            & N/A                                                            \\ \hline
\end{tabular}
}
\caption{Code size of algorithms (in bytes) for impostor detection. KS-40 means a KS test of two PED's with 40 prediction errors.}
\label{tbl_code_size}
\end{table}

==> 0800_detection_energy.tex <==
\section{Modeling Energy Consumption of Impostor Detection}
\label{sec_detection_energy}

We provide a generalized model of power consumption when the impostor detection is deployed on one/multiple hardware devices which are able to support the computation. The devices can include CPUs, GPUs and accelerators. For a system using a given set of devices ($SoD$),~\gyrefeq{eq_detection_energy} can be used to compute $E(SoD)$, which is the energy consumed within one period of sensor reading. The energy consumption of each device is computed as the sum of execution (running) energy, the idle energy and the energy to turn on ($E_{wakeup}$) and off ($E_{sleep}$) the devices.

\begin{equation}
\begin{split}
    E(SoD) = \sum_{i \in SoD} &(P_{running}(i) \times t_i 
                              + P_{idle}(i) \times (T-t_i) \\
                              &+ E_{wakeup} + E_{sleep}) \\
       SoD :~&Set~of~devices \\
         T :~&Period~of~sensor~reading
\end{split}
\label{eq_detection_energy}
\end{equation}

We then propose three principles to deploy impostor detection on a hardware system:

\bheading{Make the execution time of detection less than the period of sensor reading.} To achieve shortest latency of detection, the detection analysis should be done for each incoming reading from sensors. Hence, the computation time should be less than the period of sensor reading. It means each $t_i$ in~\gyrefeq{eq_detection_energy} should be less than the period $T$. Furthermore, if the processing on different devices are sequential, the sum of $t_i$ should be less than $T$.

\bheading{Use as less devices as possible.} Additional devices can introduce energy cost even if they are in the idle state. Moreover,~\gyrefeq{eq_detection_energy}~includes the possible energy cost to wake up devices (from idle state to running state), which can add more to the $E(SoD)$. Therefore, it is desirable to have a detection module which is versatile enough to support the full detection without subsequent processing.

\bheading{Reduce the idle power for high-performance accelerators} We consider the case when the existing high-performance accelerators are used for ML-based impostor detection. Here we ignore the functionality issue and assume the detection process can be fully supported by the accelerator (which is not true for most specialized accelerators and becomes one of the design goals of our impostor detection module). The performance-oriented accelerators, with large throughput, is possible to accomplish the computation within a short period of time. 

~\gyrefeq{eq_detection_energy}~for a single accelerator can then be reduced to~\gyrefeq{eq_detection_energy_accelerator}~if $P_{running}$ and $P_{idle}$ are of the same magnitude, which is verified in~\gyrefsec{sec_hardware_design_cost}. Given that $T$, $E_{wakeup}$ and $E_{sleep}$ can be considered a constant for a detection system, $P_{idle}$ becomes the key factor of energy consumption. Our third principle is hence to design a hardware module with enough performance and the least idle power.

\begin{equation}
\begin{split}
    E(SoD) = &P_{running} \times t_i + P_{idle} \times (T-t_i) 
              + E_{wakeup} + E_{sleep} \\
     \approx &P_{idle} \times T 
              + E_{wakeup} + E_{sleep} \\
             &(when~P_{running} \sim P_{idle}~and~t_i\ll T)
\end{split}
\label{eq_detection_energy_accelerator}
\end{equation}

We investigate the performance of detection algorithms on baseline platforms containing the general-purpose computing devices of CPU and GPU. The execution time of models giving best accuracy in~\gyrefsec{sec_sw_model} is shown in~\gyreffig{img_0800_cpugpu_time}. Two results about execution time, one for CPU platform and one for CPU-GPU platform are included for each model. The CPU platform runs the algorithms on a server with 32 Intel Xeon E5-2667 cores. We use the SciPy~\cite{scipy:jones2001scipy}~implementation of SVM, one-class SVM (OCSVM) and KS test and the TensorFlow~\cite{tensorflow:abadi2016tensorflow} CPU library for the computation of MLP and LSTM. The CPU-GPU platform uses the same server as the CPU platform and also has a NVIDIA GTX 1080Ti GPU. While the computation of MLP and LSTM can be moved to GPU by calling TensorFlow GPU library, the CPU is still needed to compute the algorithms of SVM, OCSVM and KS test.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{./figures/0800_cpugpu_time.pdf}
    \caption{Exection time of models on platforms with only CPU and both CPU and GPU}
    \label{img_0800_cpugpu_time}
\end{figure}

While the CPU-GPU platform shows the benefit to deliver better performance as expected, there are a few critical things that should be noticed in~\gyreffig{img_0800_cpugpu_time}. First, the CPU platform fails to meet the first principle to provide enough performance for real-time detection as the execution time of LSTM-based algorithms exceeds the period of sensor reading (20ms), which is shown as the solid horizontal line (black). Second, the execution time of MLP models on GPU hardly increases with regard to the model size. This means the model size is not the bottleneck of performance but it can be inferred that the initialization of TensorFlow execution contributes to a large portion of the total execution time, which can involve the loading of program and is hard to reduce. Third, the execution time of KS test is making up more than half of the whole execution time of LSTM-200-KS-OCSVM and LSTM-200-KS-Vote when the time taken by LSTM inference is greatly reduced by GPU.

These observations adds more design goals for an ideal hardware module for impostor detection.
\begin{itemize}
    \item Provide enough performance for real-time detection (in accordance with Principle 1: Make the execution time of detection less than the period of sensor reading.)
    \item Reduce the code size for fast initialization
    \item Be versatile to support the statistical test, e.g. KS test
\end{itemize}

==> tbls.tex <==
\begin{table}[]
\centering
\caption{Accuracy of regression models to recognize different users.}
\label{tbl_inst_fmt}
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real\\ User ID\end{tabular}}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Logistic\\ Regression\end{tabular}}  \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                                                          & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} \\ \hline
1                                                                                               & 61.66                    & 6.48                     & 21                            \\ \hline
2                                                                                               & 88.26                    & 5                        & 20                            \\ \hline
3                                                                                               & 66.04                    & 9.72                     & 21                            \\ \hline
4                                                                                               & 80.25                    & 6.7                      & 10                            \\ \hline
5                                                                                               & 69.19                    & 0                        & 16                            \\ \hline
6                                                                                               & 60.62                    & 19.56                    & 2                             \\ \hline
7                                                                                               & 58.35                    & 1.43                     & 16                            \\ \hline
8                                                                                               & 57.13                    & 19.44                    & 21                            \\ \hline
9                                                                                               & 76.46                    & 0                        & 16                            \\ \hline
10                                                                                              & 65.05                    & 13.27                    & 4                             \\ \hline
11                                                                                              & 77.73                    & 7.11                     & 2                             \\ \hline
12                                                                                              & 58.02                    & 7.14                     & 16                            \\ \hline
13                                                                                              & 66.38                    & 1.85                     & 21                            \\ \hline
14                                                                                              & 93.67                    & 35.6                     & 8                             \\ \hline
15                                                                                              & 72.01                    & 2.22                     & 2                             \\ \hline
16                                                                                              & 73.57                    & 6.81                     & 8                             \\ \hline
17                                                                                              & 60.3                     & 1.28                     & 14                            \\ \hline
18                                                                                              & 58.74                    & 9.26                     & 21                            \\ \hline
19                                                                                              & 53.82                    & 31.48                    & 21                            \\ \hline
20                                                                                              & 78.5                     & 3.24                     & 21                            \\ \hline
21                                                                                              & 86.06                    & 18.38                    & 14                            \\ \hline
22                                                                                              & 69.77                    & 1.33                     & 2                             \\ \hline
23                                                                                              & 64.17                    & 0                        & 16                            \\ \hline
24                                                                                              & 71.39                    & 0                        & 16                            \\ \hline
25                                                                                              & 79.78                    & 3.54                     & 4                             \\ \hline
\end{tabular}
\end{table}
























% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\label{tbl_mlp}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real\\ User\\ ID\end{tabular}}} & \multicolumn{3}{c|}{MLP-20}                                                         & \multicolumn{3}{c|}{MLP-50}                                                         & \multicolumn{3}{c|}{MLP-100}                                                        & \multicolumn{3}{c|}{MLP-500}                                                        \\ \cline{2-13} 
\multicolumn{1}{|c|}{}                                                                          & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} \\ \hline
1                                                                                               & 82.55                    & 24.5                     & 20                            & 88.86                    & 45.3                     & 13                            & 90.99                    & 54.5                     & 20                            & 90.28                    & 50                       & 20                            \\ \hline
2                                                                                               & 93.92                    & 4.5                      & 20                            & 94.7                     & 8.5                      & 20                            & 94.88                    & 10                       & 20                            & 94.16                    & 15                       & 20                            \\ \hline
3                                                                                               & 81.5                     & 5.56                     & 21                            & 88.58                    & 34.99                    & 1                             & 89.3                     & 36.12                    & 1                             & 83.99                    & 31.6                     & 1                             \\ \hline
4                                                                                               & 93.3                     & 5.26                     & 10                            & 95.37                    & 22.97                    & 10                            & 95.65                    & 16.75                    & 10                            & 95.64                    & 29.67                    & 10                            \\ \hline
5                                                                                               & 81.56                    & 4.87                     & 4                             & 83.28                    & 6.67                     & 16                            & 86.36                    & 10.53                    & 10                            & 85.07                    & 11.48                    & 10                            \\ \hline
6                                                                                               & 73.66                    & 13.33                    & 2                             & 79.62                    & 35.32                    & 15                            & 81.19                    & 34.8                     & 26                            & 80.5                     & 38                       & 26                            \\ \hline
7                                                                                               & 75.84                    & 0.95                     & 16                            & 82.92                    & 5.66                     & 9                             & 85.61                    & 5.19                     & 9                             & 84.38                    & 7.55                     & 9                             \\ \hline
8                                                                                               & 85.68                    & 40.6                     & 14                            & 89.44                    & 57.82                    & 28                            & 91.95                    & 54.5                     & 28                            & 93.17                    & 74.88                    & 28                            \\ \hline
9                                                                                               & 88.88                    & 0                        & 16                            & 90.73                    & 0                        & 16                            & 91.68                    & 0.95                     & 16                            & 90.16                    & 4.76                     & 16                            \\ \hline
10                                                                                              & 82.64                    & 17.26                    & 4                             & 86.36                    & 37.79                    & 29                            & 89.7                     & 39.63                    & 29                            & 88.81                    & 43.78                    & 29                            \\ \hline
11                                                                                              & 93.08                    & 1.78                     & 2                             & 95.43                    & 16.89                    & 2                             & 94.92                    & 15.11                    & 2                             & 94.98                    & 28.89                    & 2                             \\ \hline
12                                                                                              & 74.8                     & 15.79                    & 10                            & 85.06                    & 46.54                    & 29                            & 85.04                    & 49.6                     & 26                            & 85.63                    & 53.11                    & 10                            \\ \hline
13                                                                                              & 78.12                    & 0.93                     & 21                            & 84.5                     & 6.94                     & 21                            & 84.02                    & 17.59                    & 21                            & 84.56                    & 18.98                    & 21                            \\ \hline
14                                                                                              & 98.15                    & 56.02                    & 8                             & 98.6                     & 62.3                     & 8                             & 99.23                    & 76.96                    & 8                             & 99.05                    & 73.3                     & 8                             \\ \hline
15                                                                                              & 90.02                    & 1.33                     & 2                             & 91.1                     & 16.89                    & 2                             & 93.01                    & 25.33                    & 2                             & 91.47                    & 30.67                    & 2                             \\ \hline
16                                                                                              & 86.8                     & 3.77                     & 9                             & 89.24                    & 3.77                     & 9                             & 89.78                    & 2.83                     & 9                             & 89.07                    & 5.66                     & 9                             \\ \hline
17                                                                                              & 80.29                    & 21.99                    & 8                             & 89.65                    & 53.4                     & 8                             & 88.01                    & 43.4                     & 9                             & 88.55                    & 50                       & 9                             \\ \hline
18                                                                                              & 76.28                    & 5.78                     & 2                             & 81                       & 10.67                    & 2                             & 82.47                    & 27.56                    & 2                             & 83.4                     & 36.44                    & 2                             \\ \hline
19                                                                                              & 85.91                    & 47.59                    & 22                            & 92.95                    & 64.17                    & 22                            & 94.12                    & 57.75                    & 22                            & 93.79                    & 68.98                    & 22                            \\ \hline
20                                                                                              & 87.68                    & 11.11                    & 2                             & 90.5                     & 19.11                    & 2                             & 92.19                    & 33.78                    & 2                             & 92.45                    & 37.33                    & 2                             \\ \hline
21                                                                                              & 95.73                    & 24.79                    & 14                            & 96.6                     & 29.49                    & 14                            & 97.4                     & 41.88                    & 14                            & 96.81                    & 41.88                    & 14                            \\ \hline
22                                                                                              & 89.82                    & 4                        & 2                             & 93.44                    & 24                       & 2                             & 94.73                    & 24                       & 2                             & 95.61                    & 52                       & 2                             \\ \hline
23                                                                                              & 81.25                    & 4.29                     & 16                            & 86.5                     & 11.32                    & 9                             & 90.05                    & 44.81                    & 9                             & 89.15                    & 38.68                    & 9                             \\ \hline
24                                                                                              & 87.27                    & 0                        & 16                            & 89.21                    & 9.52                     & 16                            & 91.02                    & 24.76                    & 16                            & 89.08                    & 16.19                    & 16                            \\ \hline
25                                                                                              & 86.17                    & 5.31                     & 4                             & 88.67                    & 11.96                    & 10                            & 89.68                    & 22.01                    & 10                            & 90.61                    & 26.79                    & 10                            \\ \hline
Avg                                                                                             & 85.24                    & 12.85                    &                               & 89.29                    & 25.68                    &                               & 90.52                    & 30.81                    &                               & 90.01                    & 35.42                    &                               \\ \hline
\end{tabular}
\end{table*}














% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\label{tbl_mlptwo}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real\\ User ID\end{tabular}}} & \multicolumn{3}{c|}{MLP-50-25}                                                      & \multicolumn{3}{c|}{MLP-100-50}                                                     & \multicolumn{3}{c|}{MLP-200-100}                                                    \\ \cline{2-10} 
\multicolumn{1}{|c|}{}                                                                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} \\ \hline
1                                                                                             & 92.23                    & 59.72                    & 21                            & 93.11                    & 55                       & 20                            & 94.43                    & 60                       & 20                            \\ \hline
2                                                                                             & 95.37                    & 7                        & 20                            & 95.52                    & 10                       & 20                            & 95.61                    & 13.5                     & 20                            \\ \hline
3                                                                                             & 90.28                    & 38.43                    & 21                            & 90.92                    & 46.5                     & 1                             & 91.11                    & 45.82                    & 1                             \\ \hline
4                                                                                             & 97.45                    & 31.58                    & 10                            & 96.87                    & 25.84                    & 10                            & 96.86                    & 32.54                    & 10                            \\ \hline
5                                                                                             & 87.72                    & 11.96                    & 10                            & 87.36                    & 8.61                     & 10                            & 88.86                    & 10.05                    & 10                            \\ \hline
6                                                                                             & 81.23                    & 19.35                    & 29                            & 82.49                    & 28.57                    & 29                            & 85.22                    & 33.03                    & 15                            \\ \hline
7                                                                                             & 86.74                    & 17.45                    & 9                             & 89.34                    & 25                       & 9                             & 91.01                    & 22.64                    & 9                             \\ \hline
8                                                                                             & 89.31                    & 61.11                    & 21                            & 93.97                    & 56.87                    & 28                            & 95.24                    & 69.67                    & 28                            \\ \hline
9                                                                                             & 90.94                    & 0                        & 16                            & 91.33                    & 1.43                     & 16                            & 92.06                    & 3.33                     & 16                            \\ \hline
10                                                                                            & 90.29                    & 53.98                    & 4                             & 89.66                    & 36.41                    & 29                            & 91.53                    & 53                       & 29                            \\ \hline
11                                                                                            & 96.73                    & 16.89                    & 2                             & 96.68                    & 21.33                    & 2                             & 96.83                    & 24                       & 2                             \\ \hline
12                                                                                            & 88.18                    & 47.37                    & 10                            & 89.67                    & 46.89                    & 10                            & 92.14                    & 42.58                    & 10                            \\ \hline
13                                                                                            & 84.92                    & 14.35                    & 21                            & 83.63                    & 12.96                    & 21                            & 84.31                    & 15.74                    & 21                            \\ \hline
14                                                                                            & 98.82                    & 69.11                    & 8                             & 99.18                    & 75.92                    & 8                             & 99.22                    & 77.49                    & 8                             \\ \hline
15                                                                                            & 93.37                    & 14.22                    & 2                             & 92.64                    & 13.78                    & 2                             & 93.25                    & 25.33                    & 2                             \\ \hline
16                                                                                            & 91.17                    & 7.55                     & 9                             & 90.15                    & 9.43                     & 9                             & 89.6                     & 6.13                     & 9                             \\ \hline
17                                                                                            & 92.07                    & 57.75                    & 24                            & 92.96                    & 58.49                    & 9                             & 93.51                    & 52.83                    & 9                             \\ \hline
18                                                                                            & 85.83                    & 41.33                    & 2                             & 87.36                    & 46.22                    & 2                             & 90.3                     & 42.22                    & 2                             \\ \hline
19                                                                                            & 95.23                    & 59.89                    & 22                            & 93.69                    & 50.27                    & 22                            & 95.85                    & 49.73                    & 22                            \\ \hline
20                                                                                            & 92.75                    & 34.26                    & 21                            & 92.84                    & 37.96                    & 21                            & 94.82                    & 53.7                     & 21                            \\ \hline
21                                                                                            & 98.26                    & 62.82                    & 14                            & 98.4                     & 67.52                    & 14                            & 98.27                    & 59.83                    & 14                            \\ \hline
22                                                                                            & 93.81                    & 29.78                    & 2                             & 95.19                    & 30.22                    & 2                             & 96.73                    & 41.78                    & 2                             \\ \hline
23                                                                                            & 89.07                    & 44.34                    & 9                             & 94.34                    & 63.68                    & 9                             & 95.17                    & 71.23                    & 9                             \\ \hline
24                                                                                            & 91.53                    & 26.89                    & 9                             & 91.57                    & 31.43                    & 16                            & 92.71                    & 30                       & 16                            \\ \hline
25                                                                                            & 92.15                    & 35.89                    & 10                            & 91.9                     & 28.71                    & 10                            & 93.78                    & 39.71                    & 10                            \\ \hline
Avg                                                                                           & 91.42                    & 34.52                    &                               & 92.03                    & 35.56                    &                               & 93.14                    & 39.04                    &                               \\ \hline
\end{tabular}
\end{table*}
























% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\label{tbl_svm}
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real\\ User ID\end{tabular}}} & \multicolumn{3}{c|}{SVM}                                                            \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                                                                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{Min User} \\ \hline
1                                                                                             & 98.28                    & 60.16                    & 30                            \\ \hline
2                                                                                             & 99.91                    & 97.44                    & 13                            \\ \hline
3                                                                                             & 97.36                    & 38.18                    & 18                            \\ \hline
4                                                                                             & 99.41                    & 82.33                    & 25                            \\ \hline
5                                                                                             & 96.48                    & 34.07                    & 4                             \\ \hline
6                                                                                             & 89.15                    & 16.23                    & 12                            \\ \hline
7                                                                                             & 99.42                    & 84.91                    & 9                             \\ \hline
8                                                                                             & 97.9                     & 70.7                     & 30                            \\ \hline
9                                                                                             & 94.3                     & 0                        & 16                            \\ \hline
10                                                                                            & 96.31                    & 33.59                    & 30                            \\ \hline
11                                                                                            & 99.19                    & 80                       & 2                             \\ \hline
12                                                                                            & 98.27                    & 74.42                    & 24                            \\ \hline
13                                                                                            & 94.22                    & 35.65                    & 21                            \\ \hline
14                                                                                            & 100                      & 100                      & 1                             \\ \hline
15                                                                                            & 97.07                    & 68.02                    & 11                            \\ \hline
16                                                                                            & 94.3                     & 16.82                    & 18                            \\ \hline
17                                                                                            & 96.83                    & 23.64                    & 24                            \\ \hline
18                                                                                            & 98.97                    & 86.23                    & 11                            \\ \hline
19                                                                                            & 99.37                    & 91.44                    & 22                            \\ \hline
20                                                                                            & 98.04                    & 66.01                    & 19                            \\ \hline
21                                                                                            & 100                      & 100                      & 1                             \\ \hline
22                                                                                            & 99.97                    & 99.47                    & 22                            \\ \hline
23                                                                                            & 99.87                    & 96.55                    & 19                            \\ \hline
24                                                                                            & 98.39                    & 55.71                    & 16                            \\ \hline
25                                                                                            & 99.03                    & 72.57                    & 4                             \\ \hline
Avg                                                                                           & 97.68                    & 63.37                    & 0                             \\ \hline
\end{tabular}
\end{table}


















\begin{table}[]
\label{tbl_mlp_fft_cmp}
\caption{Accuracy of two-layer MLP models to recognize different users w/ and w/o frequency information.}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Real\\ User\\ ID\end{tabular}}} & \multicolumn{3}{c|}{MLP-Amp-200-100}                                                                                          & \multicolumn{3}{c|}{MLP-Amp-FFT-200-100}                                                                                      \\ \cline{2-7} 
\multicolumn{1}{|c|}{}                                                                          & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Min\\ User\end{tabular}} & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Min} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Min\\ User\end{tabular}} \\ \hline
1                                                                                               & 79.49                    & 7.03                     & 30                                                                      & 85.54                    & 32.03                    & 30                                                                      \\ \hline
2                                                                                               & 91.32                    & 25.35                    & 3                                                                       & 97.43                    & 78.76                    & 4                                                                       \\ \hline
3                                                                                               & 97.51                    & 81.15                    & 12                                                                      & 97.3                     & 63.87                    & 12                                                                      \\ \hline
4                                                                                               & 98.64                    & 80.91                    & 18                                                                      & 99.27                    & 92.38                    & 16                                                                      \\ \hline
5                                                                                               & 80.76                    & 28.44                    & 28                                                                      & 90.64                    & 44.55                    & 28                                                                      \\ \hline
6                                                                                               & 79.33                    & 30.41                    & 3                                                                       & 86.33                    & 22.22                    & 2                                                                       \\ \hline
7                                                                                               & 93.95                    & 45.33                    & 6                                                                       & 97.18                    & 65.33                    & 6                                                                       \\ \hline
8                                                                                               & 86.16                    & 8.87                     & 19                                                                      & 89.57                    & 10.16                    & 30                                                                      \\ \hline
9                                                                                               & 85.23                    & 35.84                    & 4                                                                       & 93.92                    & 75                       & 18                                                                      \\ \hline
10                                                                                              & 85.57                    & 15.6                     & 15                                                                      & 86.36                    & 36.36                    & 22                                                                      \\ \hline
11                                                                                              & 96.89                    & 60.78                    & 25                                                                      & 97.17                    & 79.05                    & 16                                                                      \\ \hline
12                                                                                              & 88.12                    & 10.79                    & 27                                                                      & 91.62                    & 16.59                    & 29                                                                      \\ \hline
13                                                                                              & 81.17                    & 12.33                    & 7                                                                       & 91.96                    & 33.92                    & 7                                                                       \\ \hline
14                                                                                              & 94.83                    & 21.09                    & 30                                                                      & 96.3                     & 21.48                    & 30                                                                      \\ \hline
15                                                                                              & 94.04                    & 48.85                    & 29                                                                      & 91.31                    & 27.19                    & 29                                                                      \\ \hline
16                                                                                              & 96.25                    & 46.36                    & 18                                                                      & 97.82                    & 82.27                    & 18                                                                      \\ \hline
17                                                                                              & 95.9                     & 56.8                     & 26                                                                      & 96.79                    & 77.54                    & 17                                                                      \\ \hline
18                                                                                              & 97.11                    & 53.81                    & 16                                                                      & 97.14                    & 50.48                    & 16                                                                      \\ \hline
19                                                                                              & 90.46                    & 23.44                    & 30                                                                      & 93.42                    & 31.5                     & 20                                                                      \\ \hline
20                                                                                              & 88.21                    & 3.94                     & 19                                                                      & 94.53                    & 28.08                    & 19                                                                      \\ \hline
21                                                                                              & 86.47                    & 44.34                    & 9                                                                       & 93.08                    & 71.79                    & 13                                                                      \\ \hline
22                                                                                              & 95.64                    & 63.89                    & 21                                                                      & 98.91                    & 90.74                    & 21                                                                      \\ \hline
23                                                                                              & 89.04                    & 22.66                    & 19                                                                      & 98.99                    & 92.07                    & 7                                                                       \\ \hline
24                                                                                              & 94.37                    & 56.68                    & 3                                                                       & 97.23                    & 77.03                    & 25                                                                      \\ \hline
25                                                                                              & 98.45                    & 75.19                    & 24                                                                      & 99.47                    & 91.09                    & 24                                                                      \\ \hline
Avg                                                                                             & 90.6                     & 38.4                     &                                                                         & 94.37                    & 55.66                    &                                                                         \\ \hline
\end{tabular}
\end{table}
